The Maximum Matrix Contraction Problem

In this paper, we introduce the Maximum Matrix Contraction problem, where we aim to contract as much as possible a binary matrix in order to maximize its density. We study the complexity and the polynomial approximability of the problem. Especially, we prove this problem to be NP-Complete and that every algorithm solving this problem is at most a $2\sqrt{n}$-approximation algorithm where n is the number of ones in the matrix. We then focus on efficient algorithms to solve the problem: an integer linear program and three heuristics.

==> reduction_gadgets.tex <==
\begin{figure}
\centering
\scalebox{0.7}{
		\begin{tikzpicture}
		\coordinate (O) at (0,0);

	\clip (-1,-1.25) rectangle (2.5,2.1);

    \prgrid{O}{4}{4}
    
    \prone{O}{1}{1}
    \prone{O}{3}{3}
    \draw ($(O)+(0.25,-0.3)$) node {$c_i$};
    \draw ($(O)+(1.75,-0.3)$) node {$c_i+3$};
    \draw ($(O)+(-0,0.25)$) node[anchor=east] {$l_i$};
    \draw ($(O)+(-0,0.75)$) node[anchor=east] {$l_i+1$};
    \draw ($(O)+(-0,1.25)$) node[anchor=east] {$l_i+2$};
    \draw ($(O)+(-0,1.75)$) node[anchor=east] {$l_i+3$};
    \draw ($(O)+(1,-1)$) node {$(\alpha_i)$};
    \end{tikzpicture}
		\begin{tikzpicture}
		\coordinate (O) at (0,0);
		\clip (-1,-1.25) rectangle (2.5,2.1);

    \prgrid{O}{4}{4}
    
    \prone{O}{1}{1}
    \prone{O}{2}{2}
    \draw ($(O)+(0.25,-0.3)$) node {$c_i$};
    \draw ($(O)+(1.75,-0.3)$) node {$c_i+3$};
    \draw ($(O)+(0,0.25)$) node[anchor=east] {$l_j$};
    \draw ($(O)+(0,0.75)$) node[anchor=east] {$l_j+1$};
    \draw ($(O)+(0,1.25)$) node[anchor=east] {$l_j+2$};
    \draw ($(O)+(0,1.75)$) node[anchor=east] {$l_j+3$};
    \draw ($(O)+(1,-1)$) node {$(\beta_{i,j})$};
    \end{tikzpicture}
		\begin{tikzpicture}
		\coordinate (O) at (0,0);
		\clip (-1,-1.25) rectangle (3,2.1);

    \prgrid{O}{4}{5}
    
    \prone{O}{1}{1};
    \prone{O}{2}{3};
    \prone{O}{3}{3};
    \prone{O}{3}{5};
    \prone{O}{4}{5};
    \prone{O}{4}{1};
    
    \draw ($(O)+(0.25,-0.3)$) node {$1$};
    \draw ($(O)+(0.75,-0.3)$) node {$2$};
    \draw ($(O)+(1.25,-0.3)$) node {$3$};
    \draw ($(O)+(1.75,-0.3)$) node {$4$};
    \draw ($(O)+(2.25,-0.3)$) node {$5$};
    \draw ($(O)+(-0,0.25)$) node[anchor=east] {$l_i$};
    \draw ($(O)+(-0,0.75)$) node[anchor=east] {$l_i+1$};
    \draw ($(O)+(-0,1.25)$) node[anchor=east] {$l_i+2$};
    \draw ($(O)+(-0,1.75)$) node[anchor=east] {$l_i+3$};
    \draw ($(O)+(1.25,-1)$) node {$(\gamma_i)$};
    \end{tikzpicture}
}
\caption{The three gadgets of the reduction. We do not show the 0 entries of the matrices for readability. We specify on each gadget the indexes of its lines and columns.}
   \label{fig:reduction:gadgets}
\end{figure}
